Generative Omnimatte: Learning to Decompose Video into Layers

Given a video and a set of input object masks, an omnimatte method aims to decompose the video into semantically meaningful layers containing individual objects along with their associated effects, such as shadows and reflections. Existing omnimatte methods assume a static background or accurate pose and depth estimation and produce poor decompositions when these assumptions are violated. Furthermore, due to the lack of generative prior on natural videos, existing methods cannot complete dynamic occluded regions. We present a novel generative layered video decomposition framework to address the omnimatte problem. Our method does not assume a stationary scene or require camera pose or depth information and produces clean, complete layers, including convincing completions of occluded dynamic regions. Our core idea is to train a video diffusion model to identify and remove scene effects caused by a specific object. We show that this model can be finetuned from an existing video inpainting model with a small, carefully curated dataset, and demonstrate high-quality decompositions and editing results for a wide range of casually captured videos containing soft shadows, glossy reflections, splashing water, and more.

==> figures/fig_layer_selection.tex <==
\begin{figure}
\centering
\includegraphics[trim={0 0 0 0},clip,width=\linewidth]{figures/pdfs/placeholder.pdf}
\caption{\textbf{Layer selection.} Obtain complete Omnimattes from a multi-object video.
}
\label{fig:layer_selection}
\end{figure}

==> figures/fig_object-removal_comparison_crop.tex <==
\begin{figure}
\centering
% \includegraphics[trim={0 18cm 33.5cm 0},clip,width=\linewidth]{figures/pdfs/object-removal_crop.pdf}
\includegraphics[trim={0 18cm 32.6cm 0},clip,width=\linewidth]{figures/pdfs/object-removal_crop.pdf}
\vspace{-0.6cm}
\caption{\textbf{Visual comparison on object removal.}
We compare our removal model with state-of-the-art video inpainting models~\cite{propainter,lumiere} and per-frame ObjectDrop~\cite{objectdrop}. 
Inpainting models fail to remove effects that extend beyond the provided mask boundaries. 
ObjectDrop processes video frames independently, lacking temporal information to preserve backgrounds and produce temporally coherent results. 
We encourage readers to view the supplementary material for video comparisons.
}
\label{fig:removal_comparison}
\end{figure}

==> figures/fig_omnimatte_comparison.tex <==
\begin{figure*}
\centering
% \includegraphics[trim={0 0cm 32cm 7.2cm},clip,width=0.96\linewidth]{figures/pdfs/omnimatte_comparison.pdf}
\includegraphics[trim={0 0cm 32cm 14.5cm},clip,width=0.96\linewidth]{figures/pdfs/omnimatte_comparison.pdf}
\vspace{-0.3cm}
\caption{\textbf{Visual comparisons with omnimatte methods.}
For each example, given an input video and object mask(s), we present the background layer and foreground omnimattes generated by various methods in the top and bottom rows, respectively.
Previous methods often struggle with dynamic backgrounds, leading to background dynamics being incorrectly represented in foreground layers (``kite-walk'' and ``boat-wake'').
Additionally, these methods may have difficulty completing missing pixels in fully-visible omnimattes (``kite-walk'' and ``horses'').
While Omnimatte3D~\cite{omnimatte3d} and OmnimatteRF~\cite{omnimatterf} can handle scenes with parallax effects (``horses'') better than Omnimatte~\cite{omnimatte}, the background reconstruction may still appear blurry due to imperfect 3D pose and depth estimation.
% \yaochih{Zoomed in the last example 2x so it looks blurry.}
}
\label{fig:omnimatte_comparison}
\end{figure*}

==> figures/fig_rebuttal_similar_objects.tex <==
\begin{figure}[H]
\centering
\vspace{-0.4cm}
% \includegraphics[trim={0cm 20cm 2cm 0},clip,width=\linewidth]{figures/pdfs/rebuttal_prompt.pdf}
\includegraphics[trim={0cm 34.5cm 28cm 0},clip,width=\linewidth]{figures/pdfs/rebuttal_similar_objects.pdf}
\vspace{-1cm}
\end{figure}

==> figures/fig_train_data.tex <==
\begin{figure*}
\centering
\includegraphics[trim={0.2cm 27.5cm 15cm 0.1cm},clip,width=\linewidth]{figures/pdfs/train_data.pdf}
% \includegraphics[trim={0.2cm 31cm 15cm 0.1cm},clip,width=\linewidth]{figures/pdfs/train_data_small.pdf}
\vspace{-0.6cm}
\caption{
\textbf{Training data for object and effect removal.} \todo{maybe show more examples, not overlapping with the ones in the main paper}
(a) We collect omnimatte results from existing omnimatte methods to provide examples of cause-and-effect relationships in real videos.
(b) The Tripod dataset consists of videos captured with stationary cameras, providing pseudo-examples of more complex real-world scenarios, such as water effects and dynamic backgrounds.
(c) We use the Kubric data generator~\cite{kubric} to synthesize multi-object scenes with diverse reflections and shadows.
(d) We segment objects from real videos and paste them onto target real videos~\cite{vos2019}. The trimask label for the target background is randomly assigned with either 1 or 0.5 to strengthen the model's inpainting capabilities and background preservation. 
%\erika{we can remove a row if we need space}
}
\label{fig:supp_train_data}
\end{figure*}

==> sec/5_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

\input{figures/fig_our_failures}
% The object-effect removal may not be perfect in some scenarios (Fig.~\ref{fig:our_fails}).
While our method addresses the limitations of existing approaches, it still has certain limitations.
% Firstly, our method employs a two-stage approach to decompose a video into omnimattes due to the insufficient training data for the video model to directly learn RGBA generation. \fc{Not sure we want to say this is a limitation- it's kind of our basic approach}
First, Casper requires an additional SSR step to obtain high-resolution results and the SSR model may introduce undesired noise. This noise can result in spurious background artifacts in the final omnimatte layers.

Second, omnimatte layers handle color blending (Eq.~\ref{eq:composition}) but are not designed to capture shape deformations as object effects. 
Because of this limitation, we focused on training Casper to remove color-related effects (i.e., shadows and reflections), so it may struggle to remove physical interactions with the environment (Fig.~\ref{fig:our_fails}a). % \todo{Our finetuning study suggests that, depending on the video editing use case, object removal models could be finetuned to remove different types of effects, potentially including physical interactions and lighting effects. (?)}  -- if we have such physical interaction ground-truth data?
% \yaochih{I'm not sure if physical interactions could be learned well. One case is the car smoke; even it presented in our current training data, Casper still cannot remove smokes well in testing.}
% \sarah{sg. i was thinking about how it *can* remove water effects (splashes, wakes), which are a type of physical deformation}
% \yaochih{that's a good point. Not sure if we want to clarify Casper can handle water effect such special case. Will reword "physical deformation" as "shape deformation" help separate the concept of water effects?}
% \sarah{yeah, i think "shape deformation" is maybe more accurate. or maybe just clarify that in some cases, we actually intend to preserve physical manipulations (maybe not exactly deformations though) for ghost effects, e.g., removing person but keeping umbrella / removing hands but keeping pen}

Third, the removal model may not always produce the desired outcome, particularly in challenging multi-object cases % or when removing smokes
(Fig.~\ref{fig:our_fails}b).

Fourth, the removal model may introduce undesired changes to the background, such as altering the waves in Fig.~\ref{fig:user_trimap}.
To enforce background preservation, users may specify additional regions to preserve in the trimasks. 
As shown in Fig.~\ref{fig:user_trimap}, the waves can be preserved using a coarse user-specified mask.



\input{figures/fig_user_specified_trimap}
% To address the issue, our method allows users to edit the trimap to specify the areas that they want to preserve more (Fig.~\ref{fig:user_trimap})
